A Formally Verified Procedure for Width Inference in FIRRTL

FIRRTL is an intermediate representation language for Register Transfer Level (RTL) hardware designs. In FIRRTL programs, the bit widths of many components are not specified explicitly and must be inferred during compilation. In mainstream FIRRTL compilers, such as the official compiler firtool, width inference is conducted by a compilation pass referred to as InferWidths, which may fail even for simple FIRRTL programs. In this paper, we thoroughly investigate the width inference problem for FIRRTL programs. We show that, if the constraints obtained from a FIRRTL program are satisfiable, there exists a unique least solution. Based on this result, we propose a complete procedure for solving the width inference problem. We implement it in the interactive theorem prover Rocq and prove its functional correctness. From the Rocq implementation, we extract an OCaml implementation, which is the first formally verified implementation of the InferWidths pass. Extensive experiments demonstrate that our approach can solve more instances than the official InferWidths pass in firtool, normally with high efficiency.

==> problem-bak.tex <==
%!TEX root = main.tex

\subsection{FIRRTL width constraints}

Let $X= \{x_1, \cdots, x_n\}$ be a set of variables ranging over $\natnum$, i.e. the set of natural numbers. For $n \ge 1$, let $[n]$ denote $\{1, \cdots, n\}$.

%The width inference problem of FIRRTL programs can be formulated as finding the minimum solution of a formula $\varphi$ that is a conjunction of linear inequalities of the form
%\[x_i \ge a_{0} + \sum \limits_{j \in [n]} a_{j} x_j, \]
%where $a_{0} \in \intnum$ and $a_{j} \in \natnum$. 
%%The linear inequality $x_i \ge a_{i,0} + \sum \limits_{j \in [n]} a_{i,j} x_j$ is called the inequality for $x_i$.  
%Let us use {\firlis} to denote the class of formulas $\varphi$ of this form.  

%A \emph{width term} $t$ is defined by the rules,
%\[t \eqdef x_i \mid 2^{x_i}  \mid c \mid \min(t_1,t_2) \mid t_1 + t_2,\]
%were $1 \le i \le n$ and $c \in \intnum$. Note that in width terms, the binary subtract operation is disallowed, although the minus operation in integer constants e.g. $-5$ can still be used. 

\begin{definition}[$\fwc$ constraints]
A %linear constraint $\varphi$ is called a 
FIRRTL width constraint %if it 
is a conjunction of width inequalities of the form 
\[x_i \ge \min(t_{i,1}, \cdots, t_{i, k_i}), \]
where $1 \le i \le n$ and $t_{i,1}, \cdots, t_{i, k_i}$ are width terms defined by the following rules, 
\[t \eqdef x_j \mid 2^{x_j}  \mid c \mid t + t,\]
such that $1 \le j \le n$ and $c \in \intnum$. 
\end{definition}
Note that in width terms, the binary subtract operation is disallowed, although the minus operation in integer constants e.g. $-5$ can still be used. 
For a width term $t$ and an assignment $\theta: X \rightarrow \natnum$, let $\theta(t)$ denote the value of $t$ obtained by evaluating $t$ according to the assignment $\theta$. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%removed
\hide{
\begin{definition}[{\firlis} constraints]
A %linear constraint $\varphi$ is called a 
{\firlis} constraint %if it 
is of the form $\varphi_a \wedge \varphi_l$, where 
\begin{itemize}
	\item $\varphi_a$ is a conjunction of inequalities of the form
\[x_i \ge \min(t_{i,1}, \cdots, t_{i, k_i}), \]
%such that $a_{0} \in \intnum$ and $a_{j} \in \natnum$ for $j\in[n]$,  
%
\item  $\varphi_l$ is a conjunction of inequalities of the form $b_0 \ge \sum \limits_{i \in [n]} b_i x_i$ such that $b_i \in \natnum$ for $0\leq i \leq n$. 
\end{itemize}

We say that the inequality $x_i \ge a_{0} + \sum \limits_{j \in [n]} a_{j} x_j$ \emph{constrains} $x_i$. 
\end{definition}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%removed

%\begin{remark}
%Note here for technical convenience, we additionally include the inequalities of the form $b_0 \ge \sum \limits_{i \in [n]} b_i x_i$ in {\firlis} constraints. 
%\end{remark}

For $n \ge 1$, let $\preceq_n$ denote the partial order over $\natnum^n$ such that $(u_1, \cdots, u_n) \preceq_n (v_1, \cdots, v_n)$ if for each $i \in [n]$, $u_i \le v_i$. 

For a $\fwc$ constraint $\varphi$, a solution $(u_1, \cdots, u_n)$ is said to be the \emph{minimum} solution of $\varphi$ if for each solution $(v_1, \cdots, v_n)$ of $\varphi$, $(u_1, \cdots, u_n) \preceq_n (v_1, \cdots, v_n)$.

\begin{example}
Consider the {\firlis} constraint $\varphi \equiv x_1 \ge 2 x_2 - 3 \wedge x_2 \ge 2x_1 + 1$. Then the minimum solution of $\varphi$ is $(0, 1)$. On the other hand, if $\varphi \equiv x_1 \ge 2 x_1 \wedge x_1 \ge 1$, then $\varphi$ is unsatisfiable \tl{why it is unsatisfiable?}, thus the minimum solution of $\varphi$ does not exist. 
\end{example}

%\subsection{Existence of minimum solutions of FIRLIS}

\begin{proposition}\label{prop-min-sol}
The minimum (nonnegative) solution of a satisfiable {\firlis} constraint alway exists. 
\end{proposition}

\begin{proof}
%Let $\varphi = \varphi_1 \wedge \varphi_2$ be a {\firlis} constraint such that $\varphi$ is a conjunction of inequalities of the form
%\[\bigwedge \limits_{i \in [n]} x_i \ge a_{0} + \sum \limits_{j \in [n]} a_{j} x_j,\]
%where $a_{0} \in \intnum$ and $a_{j} \in \natnum$, and $\varphi_2$ is a conjunction of the inequalities of the form $b_0 \ge \sum \limits_{i \in [n]} b_i x_i$. 

%The proposition follows from  %show 
%the following claim. 
Let $\varphi$ be a $\fwc$ constraint. 
It suffices to show that,  
%\begin{quote}
%{\bf  Claim}. 
if $(u_1, \cdots, u_n)$ and $(v_1, \cdots, v_n)$ are solutions of $\varphi$,  
then $(w_1, \cdots, w_n) = (\min(u_1, v_1), \cdots, \min(u_n, v_n))$ is also a solution of $\varphi$.
%\end{quote}
%
%\smallskip
%
%\noindent {\it Proof of the claim}. 
%
Let $I_1$ denote the set of $i \in [n]$ such that $u_i \le v_i$. Then for each $i \in I_1$, $w_i = u_i$, and for each $i \in [n] \setminus I_1$, $w_i = v_i$.

Let $x_i \ge \min(t_{i,1}, \cdots, t_{i, k_i})$ be a width inequality. 
We show that $w_i \ge \min(\theta(t_{i,1}), \cdots, \theta(t_{i, k_i}))$, where $\theta(x_i) = w_i$ for each $i \in [n]$. 

%For each $i \in [n]$, we show that $w_i \ge a_{i,0} + \sum \limits_{j \in [n]} a_{i,j} w_j$.

Evidently, for each inequality of the form $b_0 \ge \sum \limits_{i \in [n]} b_i x_i$ in $\varphi_2$, we have $b_0 \ge \sum \limits_{i \in [n]} b_i u_i \ge \sum \limits_{i \in [n]} b_i w_i$.

Let us consider an inequality of $\varphi_1$, say $x_i \ge a_{0} + \sum \limits_{j \in [n]} a_{j} x_j$ with $a_0 \in \intnum$ and $a_j \in \natnum$.
%
%Let $i \in [n]$. Then $u_i \ge a_{i,0} + \sum \limits_{j \in [n]} a_{i,j} u_j$ and $v_i \ge a_{i,0} + \sum \limits_{j \in [n]} a_{i,j} v_j$.
\begin{itemize}
\item If $u_i \le v_i$, then 
$$
\begin{array}{l c l}
w_i & = & u_i \ge a_{0} + \sum \limits_{j \in [n]} a_{j} u_j \\
& = & a_{0} + \sum \limits_{j \in I_1} a_{j} u_j + \sum \limits_{j \in [n] \setminus I_1} a_{j} u_j \\
& \ge & a_{0} + \sum \limits_{j \in I_1} a_{j} u_j + \sum \limits_{j \in [n] \setminus I_1} a_{j} v_j \\
& = & a_{0} + \sum \limits_{j \in I_1} a_{j} w_j + \sum \limits_{j \in [n] \setminus I_1} a_{j} w_j \\
& = & a_{0} + \sum \limits_{j \in [n]} a_{j} w_j. 
\end{array}
$$

\item If $u_i > v_i$, then 
$$
\begin{array}{l c l}
w_i & = & v_i \ge a_{0} + \sum \limits_{j \in [n]} a_{j} v_j \\
& = & a_{0} + \sum \limits_{j \in I_1} a_{j} v_j + \sum \limits_{j \in [n] \setminus I_1} a_{j} v_j \\
& \ge & a_{0} + \sum \limits_{j \in I_1} a_{j} u_j + \sum \limits_{j \in [n] \setminus I_1} a_{j} v_j \\
& = & a_{0} + \sum \limits_{j \in I_1} a_{j} w_j + \sum \limits_{j \in [n] \setminus I_1} a_{j} w_j \\
& = & a_{0} + \sum \limits_{j \in [n]} a_{j} w_j. 
\end{array}
$$
\end{itemize}

Therefore, $(w_1, \cdots, w_n)$ is a solution of $\varphi$. %The proof of the claim is complete. 
%From the claim, we deduce that if $\varphi$ is satisfiable, then the minimum (nonnegative) solution exists. 
\qed
\end{proof}


\hide{
The following result follows from Proposition~\ref{prop-min-sol}. 
\begin{corollary}\label{cor-min-sum}
Let $\varphi$ be a {\firlis} constraint over the variables $x_1, \cdots, x_n$. 
%conjunction of the inequalities $x_i \ge a_{0} + \sum \limits_{j \in [n]} a_{j} x_j$, where $a_{0} \in \intnum$ and $a_{j} \in \natnum$.
Let $(u_1, \cdots, u_n)$ be a solution of $\varphi$ such that $\sum \limits_{i \in I} u_i$ is the minimum among the solutions of $\varphi$.  Moreover, let $I \subseteq [n]$ and $\varphi'$ be the {\firlis} constraint that is obtained from $\varphi$ by replacing $x_i$ with $u_i$ for each $i \in I$, and $(u'_i)_{i \in [n] \setminus I}$ be the minimum solution of $\varphi'$. 
Then the solution $(v_1, \cdots, v_n)$ such that $v_i = u_i$ for each $i \in I$ and $v_i = u'_i$ for each $i \in [n] \setminus I$ is the minimum solution of $\varphi$. 
\end{corollary}

\begin{proof}
Let $(u_1, \cdots, u_n)$ be a solution of $\varphi$ such that $\sum \limits_{i \in I} u_i$ is the minimum among the solutions of $\varphi$. 
Moreover, let $I \subseteq [n]$, $\varphi'$ be the {\firlis} constraint that is obtained from $\varphi$ by replacing $x_i$ with $u_i$ for each $i \in I$, and $(u'_i)_{i \in [n] \setminus I}$ be the minimum solution of $\varphi'$. 
Let $(v_1, \cdots, v_n)$ such that $v_i = u_i$ for each $i \in I$ and $v_i = u'_i$ for each $i \in [n] \setminus I$. Then $(v_1, \cdots, v_n)$ is a solution of $\varphi$. 

Let $(w_1, \cdots, w_n)$ be the minimum solution of $\varphi$. We show that $(v_1, \cdots, v_n) = (w_1, \cdots, w_n)$. 

From the fact that  $(w_1, \cdots, w_n)$ is the minimum solution of $\varphi$, we have that for each $i \in [n]$, $w_i \le v_i$.  

Moreover, $\sum \limits_{i \in I} w_i \le \sum \limits_{i \in I} v_i = \sum \limits_{i \in I} u_i$.  From the assumption that $\sum \limits_{i \in I} u_i$ is the minimum among the solutions of $\varphi$, we deduce that $\sum \limits_{i \in I} w_i = \sum \limits_{i \in I} u_i$. From $w_i \le v_i = u_i$ for each $i \in I$, we deduce that $w_i = u_i$ for each $i \in I$. 

From $w_i = u_i$ for each $i \in I$, we deduce that $(w_i)_{i \in [n] \setminus I}$ is a solution of $\varphi'$. From the fact that $(u'_i)_{i \in [n] \setminus I}$ is the minimum solution of $\varphi'$, we deduce that $u'_i \le w_i$ for each $i \in [n] \setminus I$. 
Moreover, for each $i \in [n] \setminus I$, $w_i \le v_i = u'_i$. Therefore, for each $i \in [n] \setminus I$, $v_i = u'_i = w_i$. 

We conclude that $(v_1, \cdots, v_n) = (w_1, \cdots, w_n)$ is the minimum solution of $\varphi$. \qed
%
\end{proof}

Corollary~\ref{cor-min-sum} will be utilized to compute the minimum solution later on.
}

%%%%%%%%%%%%%%%%%%%%%%%%
\hide{
The following result follows from Proposition~\ref{prop-min-sol}. 
\begin{corollary}\label{cor-min-sum}
Let 
\[\varphi \equiv \bigwedge \limits_{i \in [n]} x_i \ge a_{i,0} + \sum \limits_{j \in [n]} a_{i,j} x_j\]
be a {\firlis} constraint, where $a_{i,0} \in \intnum$ and $a_{i,j} \in \natnum$.
If $(u_1, \cdots, u_n)$ is a solution of $\varphi$ such that $\sum \limits_{i \in [n]} u_i$ is the minimum (among the solutions of $\varphi$), then $(u_1, \cdots, u_n)$ is the minimum solution. 
\end{corollary}

\begin{proof}
Let $(u_1, \cdots, u_n)$ is a solution of $\varphi$ such that $\sum \limits_{i \in [n]} u_i$ is the minimum. Let $(v_1, \cdots, v_n)$ be a solution of $\varphi$. Then $\sum \limits_{i \in [n]} v_i \ge \sum \limits_{i \in [n]} u_i$.

From Proposition~\ref{prop-min-sol}, $(w_1, \cdots, w_n)$ with $w_i = \min(u_i, v_i)$ for each $i \in [n]$ is a solution of $\varphi$. Moreover, $\sum \limits_{i \in [n]} w_i \le \sum  \limits_{i \in [n]} u_i $. From the assumption that $\sum \limits_{i \in [n]} u_i$ is the minimum among the solutions of $\varphi$, it follows that  $\sum \limits_{i \in [n]} w_i = \sum  \limits_{i \in [n]} u_i $. Moreover, from the fact that $w_i \le u_i$ for each $i \in [n]$, we deduce that $w_i = u_i$ for each $i \in [n]$. Therefore, $u_i \le v_i$ for each $i \in [n]$. That is, $(u_1, \cdots, u_n) \preceq_n (v_1, \cdots, v_n)$. We conclude that $(u_1, \cdots, u_n)$ is the minimum solution.
\qed
\end{proof}
}
%%%%%%%%%%%%%%%%%%%%%%%%


==> problem.tex <==
%!TEX root = main.tex

%\subsection{FIRRTL width constraints}

For convenience, in this section, we assume that assume that all the variables range over $\natnum$, the set of natural numbers. Intuitively, a variable in this section represents the width of some component in a FIRRTL program. 

Throughout this section, let $X= \{x_1, \ldots, x_n\}$ denote a set of variables ranging over $\natnum$. For $n \ge 1$, let $[n]$ denote $\{1, \ldots, n\}$.

%The width inference problem of FIRRTL programs can be formulated as finding the minimum solution of a formula $\varphi$ that is a conjunction of linear inequalities of the form
%\[x_i \ge a_{0} + \sum \limits_{j \in [n]} a_{j} x_j, \]
%where $a_{0} \in \intnum$ and $a_{j} \in \natnum$. 
%%The linear inequality $x_i \ge a_{i,0} + \sum \limits_{j \in [n]} a_{i,j} x_j$ is called the inequality for $x_i$.  
%Let us use {\firlis} to denote the class of formulas $\varphi$ of this form.  

%A \emph{width term} $t$ is defined by the rules,
%\[t \eqdef x_i \mid 2^{x_i}  \mid c \mid \min(t_1,t_2) \mid t_1 + t_2,\]
%were $1 \le i \le n$ and $c \in \intnum$. Note that in width terms, the binary subtract operation is disallowed, although the minus operation in integer constants e.g. $-5$ can still be used. 

\begin{definition}[$\fwc$ constraints]
A %linear constraint $\varphi$ is called a 
FIRRTL width constraint over $X$ %if it 
is a conjunction of width inequalities of the form 
$x_i \ge \min(t_{i,1}, \ldots, t_{i, k_i})$, 
where $1 \le i \le n$ and $t_{i,1}, \ldots, t_{i, k_i}$ are width terms defined by the rules 
$t \eqdef x_j \mid 2^{x_j} \mid c \mid t + t$ such that $1 \le j \le n$ and $c \in \intnum$. 
\end{definition}
Note that in width terms, the binary subtract operation is disallowed, although the minus operation in integer constants e.g. $-5$ can still be used. 
As a result, \emph{each width term can be assumed to be of the form $a_0 + \sum \limits_{j \in [n]} a_j \tau_j$ such that $a_0 \in \intnum$ and for each $j \in [n]$, $a_j \in \natnum$, and $\tau_j = x_j$ or $2^{x_j}$}. 
For a width term $t$ and a function $\eta: X \rightarrow \natnum$, let $\eta(t)$ denote the value of $t$ obtained by evaluating $t$ according to the solution $\eta$. 
A solution of a $\fwc$ constraint $\varphi$ is a function $\eta: X \rightarrow \natnum$ such that $\eta(x_i) \ge \min(\eta(t_{i,1}), \ldots, \eta(t_{i, k_i}))$ for each width inequality $x_i \ge \min(t_{i,1}, \ldots, t_{i, k_i})$ in $\varphi$.  
For brevity, we write a solution $\eta$ as $(u_1, \ldots, u_n)$ if $\eta(x_j)=u_j$ for each $j \in [n]$. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%removed
\hide{
\begin{definition}[{\firlis} constraints]
A %linear constraint $\varphi$ is called a 
{\firlis} constraint %if it 
is of the form $\varphi_a \wedge \varphi_l$, where 
\begin{itemize}
	\item $\varphi_a$ is a conjunction of inequalities of the form
\[x_i \ge \min(t_{i,1}, \ldots, t_{i, k_i}), \]
%such that $a_{0} \in \intnum$ and $a_{j} \in \natnum$ for $j\in[n]$,  
%
\item  $\varphi_l$ is a conjunction of inequalities of the form $b_0 \ge \sum \limits_{i \in [n]} b_i x_i$ such that $b_i \in \natnum$ for $0\leq i \leq n$. 
\end{itemize}

We say that the inequality $x_i \ge a_{0} + \sum \limits_{j \in [n]} a_{j} x_j$ \emph{constrains} $x_i$. 
\end{definition}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%removed

%\begin{remark}
%Note here for technical convenience, we additionally include the inequalities of the form $b_0 \ge \sum \limits_{i \in [n]} b_i x_i$ in {\firlis} constraints. 
%\end{remark}

For $n \ge 1$, let $\preceq_n$ denote the partial order over $\natnum^n$ such that $(u_1, \ldots, u_n) \preceq_n (v_1, \ldots, v_n)$ if for each $i \in [n]$, $u_i \le v_i$. 

For a $\fwc$ constraint $\varphi$, a solution $(u_1, \ldots, u_n)$ is said to be the \emph{minimum} solution of $\varphi$ if for each solution $(v_1, \ldots, v_n)$ of $\varphi$, $(u_1, \ldots, u_n) \preceq_n (v_1, \ldots, v_n)$.

\begin{example}
\zhilin{to be cleaned}
Consider the {\firlis} constraint $\varphi \equiv x_1 \ge 2 x_2 - 3 \wedge x_2 \ge 2x_1 + 1$. Then the minimum solution of $\varphi$ is $(0, 1)$. On the other hand, if $\varphi \equiv x_1 \ge 2 x_1 \wedge x_1 \ge 1$, then $\varphi$ is unsatisfiable \tl{why it is unsatisfiable?}, thus the minimum solution of $\varphi$ does not exist. 
\end{example}

%\subsection{Existence of minimum solutions of FIRLIS}

\begin{proposition}\label{prop-min-sol}
The minimum (nonnegative) solution of a satisfiable {\firlis} constraint alway exists. 
\end{proposition}

\begin{proof}
%Let $\varphi = \varphi_1 \wedge \varphi_2$ be a {\firlis} constraint such that $\varphi$ is a conjunction of inequalities of the form
%\[\bigwedge \limits_{i \in [n]} x_i \ge a_{0} + \sum \limits_{j \in [n]} a_{j} x_j,\]
%where $a_{0} \in \intnum$ and $a_{j} \in \natnum$, and $\varphi_2$ is a conjunction of the inequalities of the form $b_0 \ge \sum \limits_{i \in [n]} b_i x_i$. 

%The proposition follows from  %show 
%the following claim. 
Let $\varphi$ be a $\fwc$ constraint. 
It suffices to show that,  
%\begin{quote}
%{\bf  Claim}. 
if $(u_1, \ldots, u_n)$ and $(v_1, \ldots, v_n)$ are solutions of $\varphi$,  
then $(w_1, \ldots, w_n) = (\min(u_1, v_1), \ldots, \min(u_n, v_n))$ is also a solution of $\varphi$. Let $\eta_1$ and $\eta_2$ denote the assignment such that $\eta_1(x_i) = u_i$ and $\eta_2(x_i)= v_i$ for each $i \in [n]$. Moreover, let $\eta$ denote the assignment such that $\eta(x_i) = w_i$ for each $i \in [n]$. 
%\end{quote}
%
%\smallskip
%
%\noindent {\it Proof of the claim}. 
%
Let $I$ denote the set of $i \in [n]$ such that $u_i \le v_i$. Then for each $i \in [n] \setminus I$, we have $u_i > v_i$. As a result,  for each $i \in I$, $w_i = u_i$, and for each $i \in [n] \setminus I$, $w_i = v_i$.

Let $i \in [n]$ and $x_i \ge \min(t_{i,1}, \ldots, t_{i, k_i})$ be a width inequality such that for each $j \in [k_i]$, $t_{i,j} = a_{i,j,0} + \sum \limits_{l \in [n]} a_{i, j, l} \tau_{i, j, l}$, where $\tau_{i, j, l} = x_l$ or $2^{x_l}$. 
In the sequel, we show that $w_i \ge \min(\eta(t_{i,1}), \ldots, \eta(t_{i, k_i}))$. 
From the arbitrariness of $i$ and width inequality, we conclude that $\eta$ is a solution of $\varphi$. 
%where $\eta(x_i) = w_i$ for each $i \in [n]$. 

%For each $i \in [n]$, we show that $w_i \ge a_{i,0} + \sum \limits_{j \in [n]} a_{i,j} w_j$.

%Evidently, for each inequality of the form $b_0 \ge \sum \limits_{i \in [n]} b_i x_i$ in $\varphi_2$, we have $b_0 \ge \sum \limits_{i \in [n]} b_i u_i \ge \sum \limits_{i \in [n]} b_i w_i$.

%Let us consider an inequality of $\varphi_1$, say $x_i \ge a_{0} + \sum \limits_{j \in [n]} a_{j} x_j$ with $a_0 \in \intnum$ and $a_j \in \natnum$.
%
%Let $i \in [n]$. Then $u_i \ge a_{i,0} + \sum \limits_{j \in [n]} a_{i,j} u_j$ and $v_i \ge a_{i,0} + \sum \limits_{j \in [n]} a_{i,j} v_j$.
Let us distinguish between the situations $u_i \le v_i$ and $u_i > v_i$.
\begin{itemize}
\item If $u_i \le v_i$, then 
$$
\begin{array}{l c l}
w_i & = & u_i \ge \min(\eta_1(t_{i,1}), \ldots, \eta_1(t_{i, k_i})) \\
& = & \min\left\{a_{i, j, 0} + \sum \limits_{l \in I} a_{i, j, l} \eta_1(\tau_{i, j, l}) + \sum \limits_{l \in [n] \setminus I} a_{i, j, l} \eta_1(\tau_{i, j, l})\ \big \vert\ j \in [k_i] \right\}\\
& \ge & \min\left\{a_{i, j, 0} + \sum \limits_{l \in I} a_{i, j, l} \eta_1(\tau_{i, j, l}) + \sum \limits_{l \in [n] \setminus I} a_{i, j, l} \eta_2(\tau_{i, j, l})\ \big \vert\ j \in [k_i] \right\} \\
& = &  \min\left\{a_{i, j, 0} + \sum \limits_{l \in I} a_{i, j, l} \eta(\tau_{i, j, l}) + \sum \limits_{l \in [n] \setminus I} a_{i, j, l} \eta(\tau_{i, j, l})\ \big \vert\ j \in [k_i] \right\} \\
& = &  \min(\eta(t_{i,1}), \ldots, \eta(t_{i, k_i})). 
\end{array}
$$
Note that the first inequality above follows from the fact that $\eta_1$ is a solution of $\varphi$ and the second inequality follows from the fact that  for each $l \in [n] \setminus I$, $u_l > v_l$, $a_{i, j, l} \ge 0$, and either $\eta_1(\tau_{i, j, l}) = \eta_1(x_l) = u_l > v_l = \eta_2(x_l) = \eta_2(\tau_{i, j, l})$ or $\eta_1(\tau_{i, j, l}) = \eta_1(2^{x_l}) = 2^{u_l} > 2^{v_l} = \eta_2(2^{x_l}) = \eta_2(\tau_{i, j, l})$.
%
\item If $u_i > v_i$, then 
$$
\begin{array}{l c l}
w_i & = & v_i \ge \min(\eta_2(t_{i,1}), \ldots, \eta_2(t_{i, k_i})) \\
& = & \min\left\{a_{i, j, 0} + \sum \limits_{l \in I} a_{i, j, l} \eta_2(x_l) + \sum \limits_{l \in [n] \setminus I} a_{i, j, l} \eta_2(x_l)\ \big \vert\ j \in [k_i] \right\}\\ \\
& \ge & \min\left\{a_{i, j, 0} + \sum \limits_{l \in I} a_{i, j, l} \eta_1(x_l) + \sum \limits_{l \in [n] \setminus I} a_{i, j, l} \eta_2(x_l)\ \big \vert\ j \in [k_i] \right\} \\
& = &  \min\left\{a_{i, j, 0} + \sum \limits_{l \in I} a_{i, j, l} \eta(x_l) + \sum \limits_{l \in [n] \setminus I} a_{i, j, l} \eta(x_l)\ \big \vert\ j \in [k_i] \right\} \\
& = & \min(\eta(t_{i,1}), \ldots, \eta(t_{i, k_i})). 
\end{array}
$$
\end{itemize}
%Therefore, $(w_1, \ldots, w_n)$ is a solution of $\varphi$. %The proof of the claim is complete. 
%From the claim, we deduce that if $\varphi$ is satisfiable, then the minimum (nonnegative) solution exists. 
\qed
\end{proof}


\hide{
The following result follows from Proposition~\ref{prop-min-sol}. 
\begin{corollary}\label{cor-min-sum}
Let $\varphi$ be a {\firlis} constraint over the variables $x_1, \ldots, x_n$. 
%conjunction of the inequalities $x_i \ge a_{0} + \sum \limits_{j \in [n]} a_{j} x_j$, where $a_{0} \in \intnum$ and $a_{j} \in \natnum$.
Let $(u_1, \ldots, u_n)$ be a solution of $\varphi$ such that $\sum \limits_{i \in I} u_i$ is the minimum among the solutions of $\varphi$.  Moreover, let $I \subseteq [n]$ and $\varphi'$ be the {\firlis} constraint that is obtained from $\varphi$ by replacing $x_i$ with $u_i$ for each $i \in I$, and $(u'_i)_{i \in [n] \setminus I}$ be the minimum solution of $\varphi'$. 
Then the solution $(v_1, \ldots, v_n)$ such that $v_i = u_i$ for each $i \in I$ and $v_i = u'_i$ for each $i \in [n] \setminus I$ is the minimum solution of $\varphi$. 
\end{corollary}

\begin{proof}
Let $(u_1, \ldots, u_n)$ be a solution of $\varphi$ such that $\sum \limits_{i \in I} u_i$ is the minimum among the solutions of $\varphi$. 
Moreover, let $I \subseteq [n]$, $\varphi'$ be the {\firlis} constraint that is obtained from $\varphi$ by replacing $x_i$ with $u_i$ for each $i \in I$, and $(u'_i)_{i \in [n] \setminus I}$ be the minimum solution of $\varphi'$. 
Let $(v_1, \ldots, v_n)$ such that $v_i = u_i$ for each $i \in I$ and $v_i = u'_i$ for each $i \in [n] \setminus I$. Then $(v_1, \ldots, v_n)$ is a solution of $\varphi$. 

Let $(w_1, \ldots, w_n)$ be the minimum solution of $\varphi$. We show that $(v_1, \ldots, v_n) = (w_1, \ldots, w_n)$. 

From the fact that  $(w_1, \ldots, w_n)$ is the minimum solution of $\varphi$, we have that for each $i \in [n]$, $w_i \le v_i$.  

Moreover, $\sum \limits_{i \in I} w_i \le \sum \limits_{i \in I} v_i = \sum \limits_{i \in I} u_i$.  From the assumption that $\sum \limits_{i \in I} u_i$ is the minimum among the solutions of $\varphi$, we deduce that $\sum \limits_{i \in I} w_i = \sum \limits_{i \in I} u_i$. From $w_i \le v_i = u_i$ for each $i \in I$, we deduce that $w_i = u_i$ for each $i \in I$. 

From $w_i = u_i$ for each $i \in I$, we deduce that $(w_i)_{i \in [n] \setminus I}$ is a solution of $\varphi'$. From the fact that $(u'_i)_{i \in [n] \setminus I}$ is the minimum solution of $\varphi'$, we deduce that $u'_i \le w_i$ for each $i \in [n] \setminus I$. 
Moreover, for each $i \in [n] \setminus I$, $w_i \le v_i = u'_i$. Therefore, for each $i \in [n] \setminus I$, $v_i = u'_i = w_i$. 

We conclude that $(v_1, \ldots, v_n) = (w_1, \ldots, w_n)$ is the minimum solution of $\varphi$. \qed
%
\end{proof}

Corollary~\ref{cor-min-sum} will be utilized to compute the minimum solution later on.
}

%%%%%%%%%%%%%%%%%%%%%%%%
\hide{
The following result follows from Proposition~\ref{prop-min-sol}. 
\begin{corollary}\label{cor-min-sum}
Let 
\[\varphi \equiv \bigwedge \limits_{i \in [n]} x_i \ge a_{i,0} + \sum \limits_{j \in [n]} a_{i,j} x_j\]
be a {\firlis} constraint, where $a_{i,0} \in \intnum$ and $a_{i,j} \in \natnum$.
If $(u_1, \ldots, u_n)$ is a solution of $\varphi$ such that $\sum \limits_{i \in [n]} u_i$ is the minimum (among the solutions of $\varphi$), then $(u_1, \ldots, u_n)$ is the minimum solution. 
\end{corollary}

\begin{proof}
Let $(u_1, \ldots, u_n)$ is a solution of $\varphi$ such that $\sum \limits_{i \in [n]} u_i$ is the minimum. Let $(v_1, \ldots, v_n)$ be a solution of $\varphi$. Then $\sum \limits_{i \in [n]} v_i \ge \sum \limits_{i \in [n]} u_i$.

From Proposition~\ref{prop-min-sol}, $(w_1, \ldots, w_n)$ with $w_i = \min(u_i, v_i)$ for each $i \in [n]$ is a solution of $\varphi$. Moreover, $\sum \limits_{i \in [n]} w_i \le \sum  \limits_{i \in [n]} u_i $. From the assumption that $\sum \limits_{i \in [n]} u_i$ is the minimum among the solutions of $\varphi$, it follows that  $\sum \limits_{i \in [n]} w_i = \sum  \limits_{i \in [n]} u_i $. Moreover, from the fact that $w_i \le u_i$ for each $i \in [n]$, we deduce that $w_i = u_i$ for each $i \in [n]$. Therefore, $u_i \le v_i$ for each $i \in [n]$. That is, $(u_1, \ldots, u_n) \preceq_n (v_1, \ldots, v_n)$. We conclude that $(u_1, \ldots, u_n)$ is the minimum solution.
\qed
\end{proof}
}
%%%%%%%%%%%%%%%%%%%%%%%%


==> procedure-exp.tex <==
%!TEX root = main.tex

In this section, we present a complete procedure to solve the width inference problem, that is, to decide the satisfiability of {\firlis} constraints and compute the minimum solution for the satisfiable constraints. 

Throughout this section, let $X= \{x_1, \cdots, x_n\}$ denote a set of variables ranging over $\natnum$.
A width inequality $x_i \ge t$ for $i \in [n]$ is called an inequality for $x_i$. 

A {\firlis} constraint is a conjunction of inequalities of the form $x \ge \min(t_1, \cdots, t_k)$. Because $x \ge \min(t_1, \cdots, t_k)$ is equivalent to $\bigvee \limits_{i \in [k]} x \ge t_i$, it follows that  a {\firlis} constraint can be rewritten into a disjunctive normal form, that is, of the form $\bigvee \limits_{i \in [m]} \bigwedge \limits_{j \in [m'_i]} z_{i,j } \ge t_{i,j }$, where $z_{i,j} \in X$ and $t_{i, j}$ defined by the rules $t \eqdef x \mid 2^x \mid c \mid t+t$, where $c \in \intnum$. A formula $\bigvee \limits_{i \in [m]} \bigwedge \limits_{j \in [m'_i]} z_{i,j } \ge t_{i,j }$ is satisfiable iff any of $\bigwedge \limits_{j \in [m'_i]} z_{i,j } \ge t_{i,j }$ is satisfiable, moreover the minimum solution of $\bigvee \limits_{i \in [m]} \bigwedge \limits_{j \in [m'_i]} z_{i,j } \ge t_{i,j }$ is the minimum among the minimum solutions of $\bigwedge \limits_{j \in [m'_i]} z_{i,j } \ge t_{i,j }$ for $i \in [m]$. 
As a result, it is sufficient to show how to solve the width inference problem for the conjunctions of width inequalities of the form $z \ge t$ such that $z \in X$ and $t$ is defined by the rules $t \eqdef x \mid 2^x \mid c \mid t+t$.

In the rest of this section, \emph{when we mention a {\firlis} constraint, we mean a conjunction of width inequalities of the form $z \ge t$ such that $z \in X$ and $t$ is defined by the rules $t \eqdef x \mid 2^x \mid c \mid t+t$}. 

The procedure utilizes a concept of dependency graphs. 


%We now present a procedure to compute the minimum solution of a {\firlis} constraint. The procedure utilizes the concept of dependency graphs. 
\begin{definition}[Dependency graph]
Let $\varphi$ be a {\firlis} constraint over $X$ and $B \in \natnum$ such that for every $i \in [n]$, the number of inequalities for $x_i$ is at most $B$. For each $i \in [n]$, let us assign a label $l \in [B]$ to each inequality for $x_i$. For convenience, we write an equality $x_i \ge a_0 + \sum \limits_{j \in [m]} a_j \tau_j$ of label $l$ as $l: x_i \ge a_0 + \sum \limits_{j \in [m]} a_j \tau_j$, where $\tau_j$ is either $x_{i'}$ or $2^{x_{i'}}$ for some $i' \in [n]$.
The dependency graph of $\varphi$, denoted by $G_\varphi$, is defined as $(V_\varphi, E_\varphi)$, where $V_\varphi=X$ and $E_\varphi \subseteq V_\varphi \times [B] \times \natnum \times \{0, 1\} \times V_\varphi$ comprises the edges $(x_i, l, a_j, b_j, x_{i'})$ such that $\varphi$ contains an inequality $l: x_i \ge a_0 + \sum \limits_{j \in [m]} a_j \tau_j$ with $a_j > 0$ and $\tau_j = x_{i'}$ or $2^{x_{i'}}$, moreover, $b_j = 1$ iff $\tau_j = 2^{x_{i'}}$. 
\end{definition}
Note that $G_\varphi$ is an edge-labeled and edge-weighted directed graph, that is, in an edge $(x_i, l, a_j, b_j, x_{i'})$, $(l, b_j)$ is seen as its label and $a_j$ is seen as its weight.  

\begin{example}
\end{example}

%In the sequel, we shall present a procedure to decide the satisfiability of {\firlis} constraints and compute the minimum solutions for satisfiable formulas. 

We are ready to present the procedure. 

Let us first consider the special cases that the dependency graphs are acyclic or strongly connected. Later on, we shall consider the more general case. 

\paragraph*{$G_\varphi$ is acyclic.} We compute the minimum solution $(u_1, \cdots, u_n)$ as follows.  
\begin{enumerate}
\item Compute a topological sorting of $G_\varphi$, say $x_{i_1}, \cdots, x_{i_n}$ (This means that the edges can only go from $x_{i_j}$ to $x_{i_{j'}}$ with $j < j'$).
%
\item Each inequality for $x_{i_n}$ is of the form $x_{i_n} \ge a_{0}$, since it does not depends on the other variables. 
Let $u_{i_n}$ denote the maximum of these $a_0$ and $0$. 
%(Without loss of generality, we assume that there is at least such $a_0$, since we can always add the inequality $x_{i_n} \ge 0$.) 

\item Let $j := n$. We iterate the following procedure to compute $u_{i_j}$'s, until $j = 1$.
\begin{enumerate}
%\item Let $u_{i_j}$ be $\max(a'_{i_j,0},0)$. 
\item Replace each occurrence of $x_{i_j}$ in the right-hand sides of the inequalities for $x_{i_1}, \cdots, x_{i_{j-1}}$ by $u_{i_j}$ and simplify the resulting expressions (by evaluating the subexpressions involving only the constants). Then each inequality for $x_{i_{j-1}}$ is of the form $x_{i_{j-1}} \ge a_0$. Let $u_{i_{j-1}}$ be the maximum of these constants $a_0$ and $0$. 
%Let $\bigwedge \limits_{j' \in [j-1]} x_{i_{j'}} \ge a'_{i_{j'}, 0} + \sum \limits_{j'' \in [j-1]} a'_{i_{j'}, j''} x_{j''}$ be the resulting constraint. (In particular, in the inequality for $i_{j-1}$, we have $a'_{i_{j-1}, j''} = 0$ for each $j'' \in [j-1]$.)
\item Let $j := j-1$.
\end{enumerate}
%
\end{enumerate}

\paragraph*{$G_\varphi$ is strongly connected.} We first prove the following result. 

\begin{proposition}\label{prop-g-1}
Suppose that $G_\varphi$ is strongly connected. If $G_\varphi$ contains two distinct edges out of some vertex $x_i$ of the same label or one edge $(x_i, l, a, b, x_j)$ such that $a > 1$ or $b=1$, then there is a constant $C \in \natnum$ such that  the values of  the variables in every solution of $\varphi$ are bounded by $C$. 
\end{proposition}
As a result, if $G_\varphi$ satisfies the conditions in Proposition~\ref{prop-g-1}, then the number of nonnegative solutions of $\varphi$ is finite and the minimum solution can be computed by an exhaustive searching. 

\begin{proof}
Suppose that $G_\varphi$ is strongly connected. 

Let us introduce a notation first. 

Suppose that $\pi = (z_0, l_1, a_1, b_1, z_1)  (z_1, l_2, a_2, b_2, z_2) \cdots (z_{m-1}, l_m, a_m, b_m, z_m)$ is a path in $G_\varphi$. We define $Ineq_\pi$, the inequality for $\pi$, as follows: For each $r \in [m]$, let the inequality for $z_{r-1}$ labeled by $l_r$ be $z_{r-1} \ge a'_{r,0} + \sum \limits_{j' \in [n]} a'_{r, j'} \tau_{r, j'}$. Then $Ineq_\pi$ is defined as $Ineq_m$, where $Ineq_1, \cdots, Ineq_m$ are computed inductively as follows. 
\begin{itemize}
\item Let $Ineq_1$ be $z_{0} \ge a'_{1,0} + \sum \limits_{j' \in [n]} a'_{1, j'} \tau_{1, j'}$. 
%
\item For each $r: 2 \le r \le m$, let $Ineq_{r}$ be obtained from $Ineq_{r-1}$ by replacing each occurrence of $z_{r-1}$ in the right-hand side of $Ineq_{r-1}$ with $a'_{r,0} + \sum \limits_{j' \in [n]} a'_{r, j'} \tau_{r, j'}$ and simplifying the resulting inequality.
Note that nested exponential terms may be introduced during the construction of $Ineq_1, \cdots, Ineq_m$. 
\end{itemize}
By an induction on $r$, we can show that $Ineq_r$ is $z_0 \ge  c_0 + \sum \limits_{j' \in [m']} c_{j'} t_{j'}$ such that
\begin{itemize}
\item $c_0 \in \intnum$, 
% 
\item for each $j' \in [m']$,  
\begin{itemize}
\item either $c_{j'} \ge 1$ is a natural number and $t_{j'} = x_j$ for some $j \in [n]$, 
%
\item or $c_{j'} > 0$ is a rational number and $t_{j'}$ is a product of exponential terms of the form $2^{x_j}$, $2^{2^{x_j}}$, $\cdots$, for $j \in [n]$,
\end{itemize}
%
\item there is $j' \in [m']$ such that $z_r$ occurs in $t_{j'}$, moreover, if $a_{r'} > 1$ or $b_{r'} = 1$ for some $r': 1 \le r' < r$, then either $c_{j'} \ge 2$ and $t_{j'} = z_r$ or $t_{j'}$ is a product of exponential terms. 
\end{itemize}
For instance, an inequality $z_0 \ge -1 + 2x_j + 2^{-1} 2^{x_k}$ may be obtained from $z_0 \ge z_1$ by replacing $z_1$ with $2x_j + 2^{x_k -1} -1 $ if the inequality for $z_1$ labeled by $l_2$ is $z_1 \ge 2x_j + 2^{x_k -1}-1$.
%Then the inequality $Inez_m$ is of the form $z_0 \ge c_0 + \sum \limits_{j' \in [n]} c_{j'} x_{j'}$. 

\smallskip
\noindent \emph{Case that $G_\varphi$ contains an edge $(x_i, l, a, b, x_j)$ with $a > 1$ or $b=1$}.
\smallskip

Take an arbitrary vertex $x_k$. Then there is a path $\pi_1$ from $x_k$ to $x_i$, and a path $\pi_2$ from $x_j$ to $x_k$, since $G_\varphi$ is strongly connected. Therefore, the path $\pi_0$ obtained by concatenating $\pi_1$, $(x_i, l, a, b, x_j)$, and $\pi_2$ is a cycle from $x_k$ to $x_k$. 
Let $Ineq_{\pi_0}$ be $x_k \ge c_0 + \sum \limits_{j' \in [m']} c_{j'} t_{j'}$. 
Then there is $j'_0 \in [m']$ such that $x_k$ occurs in $t_{j'_0}$, moreover, either $c_{j'_0} \ge 2$ and $t_{j'_0} = x_k$ or $t_{j'_0}$ is a product of exponential terms.
\begin{itemize}
\item If $c_{j'_0} \ge 2$ and $t_{j'_0} = x_k$, then $-c_0 \ge (c_{j'_0}-1) x_k + \sum \limits_{j' \in [m'] \setminus\{j'_0\}} c_{j'} t_{j'}$. This means that if $\varphi$ is satisfiable, then we must have $-c_0 \ge 0$ and the value of $x_k$ is bounded by $-c_0$. 
%
\item If $t_{j'_0} $ is a product of exponential terms, then $-c_0 - c_{j'_0} t_{j'_0} + x_k \ge \sum \limits_{j' \in [m'] \setminus \{j'_0\}} c_{j'} t_{j'}$. If $\varphi$ is satisfiable, then it must be the case that $-c_0 - c_{j'_0} t_{j'_0} + x_k \ge 0$. Because $t_{j'_0}$ is a product of exponential terms and it contains a term of the form $2^{x_k}$, $2^{2^{x_k}}$, $\cdots$, it follows that the number of values of $x_k$ so that $-c_0 - c_{j'_0} t_{j'_0} + x_k \ge 0$ (equivalently, $ c_{j'_0} t_{j'_0} - x_k \le c_0$) is bounded by some constant. As a result, if $\varphi$ is satisfiable, then the value of $x_k$ is bounded by some constant. 
%As a result, there is $C \ge 0$ such that $C \ge -c_0 - c_{j'_0} t_{j'_0} + x_k$ for every possible assignments of the variables in $-c_{j'_0} t_{j'_0} + x_k$.
%Then for each $n': 0 \le n' \le C$, $-c_0   \ge c_{j'_0} t_{j'_0}[n'/x_k] - n' + \sum \limits_{j' \in [m'] \setminus \{j'_0\}} c_{j'} t_{j'}$
\end{itemize}

%
%Let $\pi_0 = (z_0, l_1, a_1, z_1)  (z_1, l_2, a_2, z_2) \cdots (z_{m-1}, l_m, a_m, z_m)$, where $z_0 = z_m = x_k$. Moreover, for each $r \in [m]$, let the inequality of $z_{r-1}$ labeled by $l_r$ be $z_{r-1} \ge b_{r-1,0} + \sum \limits_{j' \in [n]} b_{r-1, j'} x_{j'}$. Then we compute the equalities $Ineq_r$ for $r \in [m]$ inductively as follows: Let $Ineq_1$ be $z_{0} \ge b_{0,0} + \sum \limits_{j' \in [n]} b_{0, j'} x_{j'}$. For each $r \in [m-1]$, $Ineq_{r+1}$ is obtained from $Ineq_{r}$ by replacing $z_{r}$ with  $b_{r,0} + \sum \limits_{j' \in [n]} b_{r, j'} x_{j'}$ and simplifying the resulting inequality. 
%Then the inequality $Ineq_m$ is of the form $z_0 \ge c_0 + \sum \limits_{j' \in [n]} c_{j'} x_{j'}$. From the inductive computation of $Ineq_m$ and the fact that $z_0 = z_m = x_k$, we know that $c_k = \prod_{j' \in [m]} a_{j'}$.  
%Because $(x_i, l, a, x_j)$ is a path on $\pi_0$ and $a > 1$, we deduce that $c_k > 1$. 

\smallskip
\noindent \emph{Case that $G_\varphi$ contains two distinct edges out of the same vertex, say $e_1 = (x_i, l, a_1, b_1, x_{j_1})$ and $e_2 = (x_i, l, a_2, b_2, x_{j_2})$}.
\smallskip

We can assume that for each edge $(x_{i'}, l, a, b, x_{j'})$ of $G_\varphi$, we have $a = 1$ and $b=0$. Otherwise, we can utilize the arguments in the previous case to finish the proof. 

It follows that $j_1 \neq j_2$ since $e_1$ and $e_2$ are two distinct edges. 

%Let us first consider the case that $G_\varphi$ contains two distinct edges out of some vertex $x_i$ of the same label, say $(x_i, l, a_1, b_1, x_{j_1})$ and $(x_i, l, a_2, b_2, x_{j_2})$ (where $a_1, a_2 \ge 1$ and $j_1 \neq j_2$). 
%Let the inequality for $x_i$ labeled by $l$ be $x_i \ge a'_0 + \sum \limits_{j' \in [n]} a'_{j'} \tau_{j'}$. Then $a'_{j_1} = a_1$, $a'_{j_2} = a_2$, moreover, $\tau_{j_1} = 2^{x_{j_1}}$ iff $b_{j_1} = 1$, and $\tau_{j_1} = 2^{x_{j_2}}$ iff $b_{j_2} = 1$. 
Take an arbitrary vertex $x_k$ in $G_\varphi$. Then there is a simple path $\pi_0$ from $x_k$ to $x_i$. Moreover, there are simple paths $\pi_1$ and $\pi_2$ from $x_{j_1}$ to $x_k$ and from $x_{j_2}$ to $x_k$ respectively. Let $\pi'_1$ be the concatenation of $\pi_0$, $e_1$, and $\pi_1$. Then $\pi'_1$ is a path from $x_k$ to $x_k$. 
%Similarly, let $\pi'_2$ be the concatenation of $\pi_0$, $(x_i, l, a_2, b_2, x_{j_2})$, and $\pi_2$. Then $\pi'_2$ is another path from $x_k$ to $x_k$. 
Let $Ineq_{\pi'_1}$ be $x_k \ge c_0 + \sum \limits_{j \in [n]} c_{j} x_j$. Then $c_k \ge 1$.
We distinguish between whether $\pi_1$ passes $x_{j_2}$ or not. (By passing, we mean that $\pi_1$ contains $x_{j_2}$ and $x_{j_2} \neq x_k$.) 
\begin{itemize}
\item If $\pi_1$ does not pass $x_{j_2}$, then $x_{j_2}$ occurs in $Ineq_{\pi'_0 \concat e_1}$ and remains there until $Ineq_{\pi'_1}$ is computed (where $\pi'_0 \concat e_1$ is the concatenation of $\pi'_0$ and $e_1$). 
\begin{itemize}
\item If $j_2 = k$, then we have $c_{k} \ge 2$. (Intuitively, $x_{j_1}$ produces at least one $x_k$ in $Ineq_{\pi_1}$, which, together with $x_{j_2} = x_k$, produces at least two $x_k$ in $Ineq_{\pi'_1}$.) Therefore, $-c_0 \ge (c_k-1)x_k+ \sum \limits_{j \in [n] \setminus \{k\}} c_{j} x_j$. If $\varphi$ is satisfiable, then $-c_0 \ge 0$ and the value of $x_k$ is bounded by $-c_0$.
\item Otherwise, we have $c_{j_2} \ge 1$. Let $Ineq_{\pi_2}$ be $x_{j_2} \ge d_0 + \sum \limits_{j \in [n]} d_{j} x_j$. Then $d_k \ge 1$ and 
\[
\begin{array}{l l l }
x_k & \ge & c_0 + \sum \limits_{j \in [n]} c_{j} x_j \\
& \ge & c_0 + \sum \limits_{j \in [n] \setminus \{j_2\}} c_j x_j + c_{j_2} (d_0 + \sum \limits_{j \in [n]} d_{j} x_j)\\
& = &  (c_0+c_{j_2} d_0)  + \sum \limits_{j \in [n] \setminus \{j_2\}} (c_j + c_{j_2} d_j) x_j + c_{j_2} d_{j_2} x_{j_2}. 
\end{array}
\] 
From $c_k \ge 1$, $c_{j_2} \ge 1$ and $d_k \ge 1$, we deduce that $c_k + c_{j_2} d_k \ge 2$. As a result, 
\[ -(c_0+c_{j_2} d_0)  \ge (c_k + c_{j_2} d_k - 1)x_k + \sum \limits_{j \in [n] \setminus \{j_2, k\}} (c_j + c_{j_2} d_j) x_j + c_{j_2} d_{j_2} x_{j_2}. \]
\end{itemize}
If $\varphi$ is satisfiable, then $-(c_0+c_{j_2} d_0) \ge 0$ and the value of $x_k$ is bounded by $-(c_0+c_{j_2} d_0)$.
%
\item If $\pi_1$ passes $x_{j_2}$, then let $\pi_1 = \pi''_1 \concat \pi'''_1$ such that $\pi''_1$ is the prefix of $\pi_1$ that goes from $x_{j_1}$ to $x_{j_2}$. Let $Ineq_{\pi_0 \concat e_1}$ be $x_{k} \ge d_0 + \sum \limits_{j \in [n]} d_{j} x_j$. Then $d_{j_1} \ge 1$ and $d_{j_2} \ge 1$. Moreover, let $Ineq_{\pi''_1}$ be $x_{j_1} \ge d'_0 + \sum \limits_{j \in [n]} d'_{j} x_j$. Then $d'_{j_2} \ge 1$. As a result, $Ineq_{\pi_0 \concat e_1 \concat \pi''_1}$ is 
\[
\begin{array}{l l l}
x_k & \ge & d_0 + \sum \limits_{j \in [n] \setminus \{j_1\}} d_{j} x_j + d_{j_1} (d'_0 + \sum \limits_{j \in [n]} d'_{j} x_j)\\
& \ge & (d_0 + d_{j_1} d'_0) + \sum \limits_{j \in [n] \setminus \{j_1\}} (d_{j} + d_{j_1}d'_j) x_j  + d_{j_1} d'_{j_1} x_{j_1}.
\end{array}
\]
Then $d_{j_2} + d_{j_1}d'_{j_2} \ge 2$.
Consequently, in $Ineq_{\pi'_1} = Ineq_{\pi_0 \concat e_1 \concat \pi''_1 \concat \pi'''_1}$, which is obtained from $Ineq_{\pi_0 \concat e_1 \concat \pi''_1}$ by replacing $x_{j_2}$ with the right-hand side of $Ineq_{\pi'''_1}$, the coefficient of $x_{k}$ is at least two, since the coefficient of $x_{j_2}$ in $Ineq_{\pi_0 \concat e_1 \concat \pi''_1}$ is $d_{j_2} + d_{j_1}d'_{j_2} \ge 2$.
\end{itemize}
\qed
\end{proof}

%Therefore, from Proposition~\ref{prop-g-1}, if $G_\varphi$ contains an edge of weight greater than $1$ or two distinct edges out of some vertex $x_i$ of the same label, then the number of solutions satisfying $\varphi$ is finite and we can find the minimum solution by guessing the solution candidates from the least to the greatest one by one and check whether they are indeed solutions. 

In the sequel, let us assume that each edge $(x_i, a, b, x_j)$ in $G_\varphi$ satisfies that $a = 1$ and $b=0$, moreover, all the edges out of the same vertex have mutually distinct labels. Then each inequality in $\varphi$ is of the form $x_i \ge c + x_j$ for some $c \in \intnum$.

Then for each vertex $x_i$, we guess all the simple cycles that involve $x_i$ and do the following for each such simple cycle.  
Let $C = x_{l_1} \cdots x_{l_r} x_{l_{r+1}}$ be a simple cycle where $l_{r+1} = l_1 = i$. We compute $u_{C, l_1}, \cdots, u_{C, l_r}$ as follows. 
 For each $j' \in [r]$, let the inequality corresponding to the $j'$-th edge of $C$ be $x_{l_{j'}} \ge a_{l_{j'}} + x_{l_{(j' \bmod r)+1}}$. 
%$$x_{l_{j'}} \ge a_{l_{j'},0} + \sum \limits_{j'' \in I_1} a_{l_{j'}, j''} u_{j''} + \sum \limits_{x_{j''} \in V(C_i) \setminus V(C')} a_{l_{j'}, j''}  u_{j''} + x_{l_{(j' \bmod r)+1}}.$$ 
%
%For each $j' \in [r]$, let $b_{l_{j'}}$ denote 
%$$a_{l_{j'},0} + \sum \limits_{j'' \in I_1} a_{l_{j'}, j''} u_{j''} + \sum \limits_{x_{j''} \in V(C_i) \setminus V(C')} a_{l_{j'}, j''}  u_{j''}.$$ 
%
%Then $x_{l_{j'}} \ge b_{l_{j'}} + x_{l_{(j' \bmod r)+1}}$ for each $j' \in [r]$.
\begin{itemize}
\item If $\sum \limits_{j' \in [r]} a_{l_{j'}} > 0 $, then $\varphi$ is unsatisfiable. 
%
\item Otherwise, for each $j' \in [r]$, let $u_{C, l_{j'}} := \max(0, a_{l_{j'}}, a_{l_{j'}}+ a_{l_{j'+1}}, \cdots, (a_{l_{j'}} + \cdots + a_{l_{((j'+r-2) \bmod r)+1}})$. 
%(From $\sum \limits_{j' \in [r]} a_{l_{j'}} \le 0$, it is unnecessary to include $\sum \limits_{j' \in [r]} a_{l_{j'}}$ here.)
\end{itemize}
Finally, for each $i \in [n]$, we compute the minimum solution as $(u_1, \cdots, u_n)$ such that for each $i \in [n]$, $u_i$ is the maximum of all $u_{C, l_1}$ such that $C = x_{l_1} \cdots x_{l_r} x_{l_{r+1}}$ is a simple cycle where $l_{r+1} = l_1 = i$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hide{
Since the in-degree of each vertex in $G_\varphi$ is at least one, each variable $x_i$ occurs at least once in the right-hand sides of the inequalities, that is, there is at least one equality for some variable $x_{i'}$, say $x_{i'} \ge a_0 + \sum \limits_{j \in [n]} a_j x_j$, such that $a_i > 0$. For each $i \in [n]$, let $a'_i$ denote the sum of these coefficients $a_i$ in the right-side hands of the inequalities. 
Let $I_1$ denote the set of $i \in [n]$ such that $a'_i > 1$. 

It is easy to see that the sum of the left-hand sides of the inequalities for all the variables is greater than or equal to the sum of the right-hand sides of these inequalities, that is, 
$$\sum \limits_{i \in [n]} x_i \ge \sum \limits_{i \in [n]} \left(a_{i,0} + \sum \limits_{j \in [n]} a_{i,j} x_j \right) \ge \sum \limits_{i \in [n]} a_{i,0} + \sum \limits_{i \in [n]} \left(\sum \limits_{j \in [n]} a_{j, i} \right) x_i.$$

Then 
$$0 \ge  \sum \limits_{i \in [n]} a_{i,0} + \sum \limits_{i \in I_1} \left(\sum \limits_{j \in [n]} a_{j, i} \right) x_i.$$
That is, 
$$- \sum \limits_{i \in [n]} a_{i,0}  \ge  \sum \limits_{i \in I_1} \left(\sum \limits_{j \in [n]} a_{j, i} \right) x_i.$$

If $- \sum \limits_{i \in [n]} a_{i,0} < 0$, then $\varphi$ is unsatisfiable. Otherwise, we can enumerate the tuples $(u_i)_{i \in I_1}$ such that 
$$- \sum \limits_{i \in [n]} a_{i,0}  \ge  \sum \limits_{i \in I_1} \left(\sum \limits_{j \in [n]} a_{j, i} \right) u_i.$$
Let $\valset_{I_1}$ denote the set of such tuples $(u_i)_{i \in I_1}$.

From Corollary~\ref{cor-min-sum}, we can compute the minimum solution of $\varphi$ as follows: 
We enumerate the tuples $(u_i)_{i \in I_1}$ in $\valset_{I_1}$ one by one, in the order that $\sum \limits_{i \in I_1} u_i$ is nondecreasing. For each enumerated tuple $(u_i)_{i \in I_1}$, replace each occurrence of $x_i$ for $i \in I_1$ in the right-hand side of the inequalities by $u_i$ and obtain 
%
\[\varphi' \equiv \bigwedge \limits_{i \in I_1} u_i \ge a_{i,0} + \sum \limits_{j \in I_1} a_{i, j} u_j + \sum \limits_{j \in [n] \setminus I_1} a_{i, j} x_j \wedge \bigwedge \limits_{i \in [n] \setminus I_1} x_i \ge a_{i,0} + \sum \limits_{j \in I_1} a_{i, j} u_j + \sum \limits_{j \in [n] \setminus I_1} a_{i, j} x_j.
\]
If the minimum solution $(u_j)_{j \in [n] \setminus I_1}$ is found for $\varphi'$, then $(u_j)_{j \in [n]}$ is the minimum solution of $\varphi$ and the computation stops. If for each enumerated tuple from $\valset_{I_1}$, no solution is found for $\varphi'$, then $\varphi$ is unsatisfiable. 

In the sequel, let us show how to compute the minimum solution for $\varphi'$ (if it exists).

Let us first focus on 
\[
\psi  \equiv \bigwedge \limits_{i \in [n] \setminus I_1} x_i \ge a_{i,0} + \sum \limits_{j \in I_1} a_{i, j} u_j + \sum \limits_{j \in [n] \setminus I_1} a_{i, j} x_j.
\]
From the definition of $I_1$, we know that $\sum \limits_{j \in [n] \setminus I_1} a_{j, i} = 1$.  

Then the dependency graph $G_\psi$ satisfies that the in-degree of each vertex in $G_\psi$ are at most $1$. Then \emph{each connected component of $G_\psi$ is either a tree, or a tree plus one additional edge from a leaf to the root}. Let $C_1, \cdots, C_k$ be an enumeration of the connected components of $G_\psi$. 

For each $i \in [k]$, we compute a tuple $(u_j)_{x_j \in V(C_i)}$ as follows.  

\begin{itemize}
\item If $C_i$ is a tree, then we compute a tuple $(u_j)_{x_j \in V(C_i)}$ in a bottom-up way. Let $x_j \in V(C_i)$.  
\begin{itemize}
\item If $x_j$ is a leaf in $C_i$, then $x_j \ge a_{j,0} + \sum \limits_{j' \in I_1} a_{j, j'} u_{j'}$ and let $u_j := a_{j,0} + \sum \limits_{j' \in I_1} a_{j, j'} u_{j'}$.
%
\item Otherwise, $x_j \ge a_{j, 0} + \sum \limits_{j' \in I_1} a_{j, j'} u_{j'} + \sum \limits_{j' \in [n] \setminus I_1} a_{j, j'} x_{j'}$, where  $a_{j,j'} > 0$ for some $j' \in [n] \setminus I_1$. Moreover, for each $j' \in [n] \setminus I_1$ with $a_{j, j'} > 0$, $u_{j'}$ has been computed. Then  $x_j \ge a_{j, 0} + \sum \limits_{j' \in I_1} a_{j, j'} u_{j'} + \sum \limits_{j' \in [n] \setminus I_1} a_{j, j'} u_{j'}$, let $u_j = \max(0, a_{j, 0} + \sum \limits_{j' \in I_1} a_{j, j'} u_{j'} + \sum \limits_{j' \in [n] \setminus I_1} a_{j, j'} u_{j'})$.
\end{itemize}

\item If $C_i$ is a tree with one additional edge from a leaf $x_j$ to the root, then the path from the root to $x_j$ and the edge from $x_j$ to the root constitute  a simple cycle $C'$. Then for each vertex $x_{j'}$ not belonging to $C'$, we compute $u_{j'}$ as in the case that $C_i$ is a tree. Let $C' = x_{l_1} \cdots x_{l_r} x_{l_{r+1}}$ where $l_{r+1} = l_1$. Then for each $j' \in [r]$, $a_{l_{j'}, l_{(j' \bmod r)+1}} = 1$ and 
$$x_{l_{j'}} \ge a_{l_{j'},0} + \sum \limits_{j'' \in I_1} a_{l_{j'}, j''} u_{j''} + \sum \limits_{x_{j''} \in V(C_i) \setminus V(C')} a_{l_{j'}, j''}  u_{j''} + x_{l_{(j' \bmod r)+1}}.$$ 
%
For each $j' \in [r]$, let $b_{l_{j'}}$ denote 
$$a_{l_{j'},0} + \sum \limits_{j'' \in I_1} a_{l_{j'}, j''} u_{j''} + \sum \limits_{x_{j''} \in V(C_i) \setminus V(C')} a_{l_{j'}, j''}  u_{j''}.$$ 
%
Then $x_{l_{j'}} \ge b_{l_{j'}} + x_{l_{(j' \bmod r)+1}}$ for each $j' \in [r]$.
\begin{itemize}
\item If $\sum \limits_{j' \in [r]} b_{l_{j'}} > 0 $, then $\varphi'$ is unsatisfiable. 
%
\item Otherwise, for each $j' \in [r]$, let $u_{l_{j'}} := \max(0, b_{l_{j'}}, b_{l_{j'}}+ b_{l_{j'+1}}, \cdots, b_{l_{j'}} + \cdots + b_{l_{(j'+r-3) \bmod r+1}})$.
\end{itemize}
\end{itemize}

Therefore, a tuple $(u_j)_{j \in [n] \setminus I_1}$ has been computed.
\begin{itemize}
\item If $u_i < a_{i,0} + \sum \limits_{j \in I_1} a_{i, j} u_j + \sum \limits_{j \in [n] \setminus I_1} a_{i, j} u_j$ for some $i \in I_1$, then $\varphi'$ is unsatisfiable. 
%
\item Otherwise, $(u_j)_{j \in [n] \setminus I_1}$ is the minimum solution of $\varphi'$.
\end{itemize}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph*{More general case.} Suppose that $G_\varphi$ is neither acyclic nor strongly connected. 
%Therefore, $G_\varphi$ contains at least two nontrivial SCCs. 
Let $\sccgraph_{G_\varphi}$ be the SCC graph of $G_\varphi$. We compute a topological sorting of $\sccgraph_{G_\varphi}$, say $C_1, \cdots, C_k$. (If there are edges from the vertices in $C_i$ to the vertices in $C_j$, then $i < j$.) Let $j := k$.  We iterate the following procedure, until $j=1$. 
\begin{enumerate}
\item Suppose $u_{j'} \in \natnum$ has been computed for each $x_{j'} \in V(C_{j+1}) \cup \cdots \cup V(C_k)$. For each $x_{j''} \in V(C_j)$, replace each occurrence of $x_{j'} \in V(C_{j+1}) \cup \cdots \cup V(C_k)$ in the right-hand sides of the inequalities for $x_{j''}$ with $u_{j'}$. 
%For each $x_{j''} \in V(C_j)$, let the resulting inequality be $x_{j''} \ge b_0 + \sum \limits_{x_{j'} \in V(C_j)} b_{j'} x_{j'}$, where $b_{j''} \in \intnum$. 
Let $\psi_{C_j}$ be the conjunction of the resulting inequalities for $x_{j''} \in V(C_j)$.
Then we can utilize the aforementioned procedure for strongly connected graphs to compute the minimum solution $(u_{j''})_{x_{j''} \in V(C_j)}$ for $\psi_{C_j}$. If during the computation, $\psi_{C_j}$ is discovered to be unsatisfiable, then $\varphi$ is unsatisfiable and the computation stops. 
%
\item Let $j:=j-1$. 
\end{enumerate}

%\paragraph*{Complexity analysis.} It is not hard to see that the time complexity of the aforementioned procedure is polynomial in the \emph{values of the integer constants in $\varphi$} and exponential over $n$, the number of variables in $\varphi$. 
%Moreover, if $a_{i,j} \le 1$ for each $i \in [n]$ and $j \in [n]$, then the time complexity procedure is also polynomial in the number of variables in $\varphi$. 
%Moreover, since the values of these constants involved in the width inference problem are polynomial in the size of a FIRRTL program, it follows that the width inference problem can be solved in polynomial time, if each ground component occurs at most once in the right-side hand of the connect statements.  

==> proof_prop3.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}[of Proposition~\ref{prop-g-1}]
We first introduce some notations. 
\begin{definition}[Inequalities for paths]
Consider a path $\pi$ in $G_\varphi$
$$\pi = (z_0, l_1, a_1, z_1)  (z_1, l_2,a_2,  z_2)\cdots (z_{m-1}, l_m, a_m,  z_m).$$
 For each $r \in [m]$, 
let $l_r: z_{r-1} \ge a_{r,0} + \sum_{j \in [n]} a_{r, j} x_j$ be
the inequality for $z_{r-1}$ labeled by $l_r$.
The inequality for the path $\pi$, $\mathsf{Ineq}_\pi$, is defined as $\mathsf{Ineq}_m$, where $\mathsf{Ineq}_0, \ldots, \mathsf{Ineq}_m$ are defined inductively as follows: 
% \begin{description}
\begin{itemize}
\item Base: $\mathsf{Ineq}_0$ is the inequality $z_{0} \ge z_0$, i.e., $a_{1,0} + \sum_{j \in [n]} a_{1, j} x_j$ is $z_0$.
%
\item Inductive step: For each $r\in [m]$, let $\mathsf{Ineq}_{r}$ be the inequality obtained from $\mathsf{Ineq}_{r-1}$ by replacing each occurrence of $z_{r-1}$ in the right-hand side of $\mathsf{Ineq}_{r-1}$ with $a_{r,0} + \sum_{j \in [n]} a_{r, j} x_j$ and simplifying the resulting inequality.
%Note that nested exponential terms may be introduced during the construction of $Ineq_1, \cdots, Ineq_m$. 
\end{itemize}
% \end{description}
\end{definition}
For instance, an inequality $z_0 \ge -1 + 2x_j$ may be obtained from $l_1: z_0 \ge z_1$ by replacing $z_1$ with $-1+2x_j$ if the inequality for $z_1$ labeled by $l_2$ is $z_1 \ge -1+2x_j$.

We denote by $\pi_1 \concat\pi_2$ the concatenation of two paths $\pi_1$ and $\pi_2$.

\medskip
% \noindent\underline{\bf ``Only If'' direction}.
\noindent\underline{``Only If'' direction}.
Suppose $G_\varphi$ is expansive, then $G_\varphi$ contains an edge $(x_i, l, a, x_j)$ with $a > 1$ or two distinct edges out of some vertex with the same label. 
We proceed
by a case distinction.

\smallskip
% \noindent \emph{\bf Case that $G_\varphi$ contains an edge $(x_i, l, a, x_j)$ with $a > 1$}.
\emph{\bf Case that $G_\varphi$ contains an edge $(x_i, l, a, x_j)$ with $a > 1$}:
\smallskip

Take an arbitrary vertex $x_k$ in $G_\varphi$.
Since $G_\varphi$ is strongly connected, there must exist a path $\pi_1$ from $x_k$ to $x_i$, and a path $\pi_2$ from $x_j$ to $x_k$. 
Therefore, the path $\pi=\pi_1\concat (x_i, l, a, x_j)\concat\pi_2$ %obtained by concatenating $\pi_1$, $(x_i, l, a, x_j)$, and $\pi_2$ 
forms a cycle from $x_k$ to $x_k$ in $G_\varphi$. 

Let $\mathsf{Ineq}_{\pi}$ be $x_k \ge c_0 + \sum_{j \in [n]} c_{j} x_j$. Then $c_j\in\natnum$ for $j\in [n]$ and moreover $c_k\geq 2$ because $a>1$.
From the inequality $x_k \ge c_0 + \sum_{j \in [n]} c_{j} x_j$, if $\varphi$ is satisfiable, we can deduce that:
$$-c_0 \ge (c_{k}-1) x_k + \sum_{j\in [n] \setminus\{k\}} c_{j} x_{j}\ge (c_{k}-1) x_k \ge (2-1) x_k\ge x_k\ge 0.$$

%It implies that if $\varphi$ is satisfiable, then %we must have $-c_0 \ge 0$ and 
Thus, if $\varphi$ is satisfiable, the value of $x_k$ is upper-bounded by $-c_0$. 

%there is $j'\in [n]$ such that $x_{k}$ 
%and $x_{j'}$ are, moreover, either $c_{j'_0} \ge 2$ and $t_{j'_0} = x_k$ or $t_{j'_0}$ is a product of exponential terms.
\hide{
\begin{itemize}
\item If $c_{j'_0} \ge 2$ and $t_{j'_0} = x_k$, then $-c_0 \ge (c_{j'_0}-1) x_k + \sum \limits_{j' \in [m'] \setminus\{j'_0\}} c_{j'} t_{j'}$. This means that if $\varphi$ is satisfiable, then we must have $-c_0 \ge 0$ and the value of $x_k$ is bounded by $-c_0$. 
%
\item If $t_{j'_0} $ is a product of exponential terms, then $-c_0 - c_{j'_0} t_{j'_0} + x_k \ge \sum \limits_{j' \in [m'] \setminus \{j'_0\}} c_{j'} t_{j'}$. If $\varphi$ is satisfiable, then it must be the case that $-c_0 - c_{j'_0} t_{j'_0} + x_k \ge 0$. Because $t_{j'_0}$ is a product of exponential terms and it contains a term of the form $2^{x_k}$, $2^{2^{x_k}}$, $\cdots$, it follows that the number of values of $x_k$ so that $-c_0 - c_{j'_0} t_{j'_0} + x_k \ge 0$ (equivalently, $ c_{j'_0} t_{j'_0} - x_k \le c_0$) is bounded by some constant. As a result, if $\varphi$ is satisfiable, then the value of $x_k$ is bounded by some constant. 
%As a result, there is $C \ge 0$ such that $C \ge -c_0 - c_{j'_0} t_{j'_0} + x_k$ for every possible assignments of the variables in $-c_{j'_0} t_{j'_0} + x_k$.
%Then for each $n': 0 \le n' \le C$, $-c_0   \ge c_{j'_0} t_{j'_0}[n'/x_k] - n' + \sum \limits_{j' \in [m'] \setminus \{j'_0\}} c_{j'} t_{j'}$
\end{itemize}
}

%
%Let $\pi_0 = (z_0, l_1, a_1, z_1)  (z_1, l_2, a_2, z_2) \cdots (z_{m-1}, l_m, a_m, z_m)$, where $z_0 = z_m = x_k$. Moreover, for each $r \in [m]$, let the inequality of $z_{r-1}$ labeled by $l_r$ be $z_{r-1} \ge b_{r-1,0} + \sum \limits_{j' \in [n]} b_{r-1, j'} x_{j'}$. Then we compute the equalities $Ineq_r$ for $r \in [m]$ inductively as follows: Let $Ineq_1$ be $z_{0} \ge b_{0,0} + \sum \limits_{j' \in [n]} b_{0, j'} x_{j'}$. For each $r \in [m-1]$, $Ineq_{r+1}$ is obtained from $Ineq_{r}$ by replacing $z_{r}$ with  $b_{r,0} + \sum \limits_{j' \in [n]} b_{r, j'} x_{j'}$ and simplifying the resulting inequality. 
%Then the inequality $Ineq_m$ is of the form $z_0 \ge c_0 + \sum \limits_{j' \in [n]} c_{j'} x_{j'}$. From the inductive computation of $Ineq_m$ and the fact that $z_0 = z_m = x_k$, we know that $c_k = \prod_{j' \in [m]} a_{j'}$.  
%Because $(x_i, l, a, x_j)$ is a path on $\pi_0$ and $a > 1$, we deduce that $c_k > 1$. 

\smallskip
% \noindent \emph{\bf Case that $G_\varphi$ contains two distinct edges out of the some vertex with the same label}.
\emph{\bf Case that $G_\varphi$ contains two distinct edges out of the some vertex with the same label}:
\smallskip

Let $e_1 = (x_i, l, a_1, x_{j_1})$ and $e_2 = (x_i, l, a_2, x_{j_2})$ be two distinct edges out of the vertex $x_i$ in $G_\varphi$ with the same label $l$.
We assume that for each edge $(x_{i'}, l, a, x_{j'})$ of $G_\varphi$, $a = 1$, otherwise, 
the result immediately follows from $a>1$. 

%It follows that $j_1 \neq j_2$ since $e_1$ and $e_2$ are two distinct edges. 

%Let us first consider the case that $G_\varphi$ contains two distinct edges out of some vertex $x_i$ of the same label, say $(x_i, l, a_1, b_1, x_{j_1})$ and $(x_i, l, a_2, b_2, x_{j_2})$ (where $a_1, a_2 \ge 1$ and $j_1 \neq j_2$). 
%Let the inequality for $x_i$ labeled by $l$ be $x_i \ge a'_0 + \sum \limits_{j' \in [n]} a'_{j'} \tau_{j'}$. Then $a'_{j_1} = a_1$, $a'_{j_2} = a_2$, moreover, $\tau_{j_1} = 2^{x_{j_1}}$ iff $b_{j_1} = 1$, and $\tau_{j_1} = 2^{x_{j_2}}$ iff $b_{j_2} = 1$. 
Take an arbitrary vertex $x_k$ in $G_\varphi$.
Since $G_\varphi$ is strongly connected, there must exist a simple path $\pi_0$ from $x_k$ to $x_i$, and two distinct simple paths $\pi_1$ and $\pi_2$ from $x_{j_1}$ to $x_k$ and from $x_{j_2}$ to $x_k$, respectively. Let $\pi'_1=\pi_0\concat e_1 \concat\pi_1$, 
%and $\pi'_2=\pi_0\concat e_2 \concat\pi_2$
which is a cycle from $x_k$ to $x_k$. 

%be the concatenation of $\pi_0$, $e_1$, and $\pi_1$. Then $\pi'_1$ is a cycle from $x_k$ to $x_k$. 
%Similarly, let $\pi'_2$ be the concatenation of $\pi_0$, $(x_i, l, a_2, b_2, x_{j_2})$, and $\pi_2$. Then $\pi'_2$ is another path from $x_k$ to $x_k$. 

Let $\mathsf{Ineq}_{\pi'_1}$ be $x_k \ge c_0 + \sum_{j \in [n]} c_{j} x_j$. Then $c_j\in\natnum$ for $j\in [n]$ and moreover $c_k \ge 1$.
The proof proceeds by distinguishing whether $\pi_1$ passes $x_{j_2}$ or not. (By passing, we mean that $\pi_1$ contains $x_{j_2}$ and $x_{j_2} \neq x_k$.) 
\begin{itemize}
\item If $\pi_1$ does not pass $x_{j_2}$, then $x_{j_2}$ must occur in $\mathsf{Ineq}_{\pi_0 \concat e_1}$ (since $a_2 x_{j_2}$ is a sub-term of the right-hand side of the inequality labeled by $l$) and remain therein until $\mathsf{Ineq}_{\pi_1'}$ (i.e., $\mathsf{Ineq}_{\pi_0 \concat e_1\concat \pi_1}$) is computed. 
\begin{itemize}
\item If $j_2 = k$, then we have $c_{k} \ge 2$. (Intuitively, the iterative replacement that goes through $x_{j_1}$ produces at least one $x_k$ in $\mathsf{Ineq}_{\pi'_1}$, which, together with going through $x_{j_2} = x_k$, produces at least two $x_k$ in $\mathsf{Ineq}_{\pi'_1}$.) Therefore, we get that 
if $\varphi$ is satisfiable, then
$$-c_0 \ge (c_{k}-1) x_k + \sum_{j\in [n] \setminus\{k\}} c_{j} x_{j}\ge (c_{k}-1) x_k \ge (2-1) x_k\ge x_k\ge 0.$$
Thus, if $\varphi$ is satisfiable, then the value of $x_k$ is upper-bounded by $-c_0$.
%%%%
%%%%
\item Otherwise, we have $c_{j_2} \ge 1$. Let $\mathsf{Ineq}_{\pi_2}$ be $x_{j_2} \ge d_0 + \sum_{j \in [n]} d_{j} x_j$. Then $d_k \ge 1$ and 
\[\renewcommand{\arraystretch}{1.5}
\begin{array}{l l l }
x_k & \ge & c_0 + \sum_{j \in [n]} c_{j} x_j \\
& \ge & c_0 + \sum_{j \in [n] \setminus \{j_2\}} c_j x_j + c_{j_2} (d_0 + \sum_{j \in [n]} d_{j} x_j)\\
& = &  (c_0+c_{j_2} d_0)  + \sum_{j \in [n] \setminus \{j_2\}} (c_j + c_{j_2} d_j) x_j + c_{j_2} d_{j_2} x_{j_2}. 
\end{array}
\] 
From $c_k \ge 1$, $c_{j_2} \ge 1$ and $d_k \ge 1$, we deduce that $c_k + c_{j_2} d_k \ge 2$. Hence 
\[-(c_0+c_{j_2} d_0)  \ge (c_k + c_{j_2} d_k - 1)x_k + \sum \limits_{j \in [n] \setminus \{j_2, k\}} (c_j + c_{j_2} d_j) x_j + c_{j_2} d_{j_2} x_{j_2}. \]
\end{itemize}
If $\varphi$ is satisfiable, then $-(c_0+c_{j_2} d_0) \ge 0$ and the value of $x_k$ is upper-bounded by $-(c_0+c_{j_2} d_0)$.
%
\item If $\pi_1$ passes $x_{j_2}$, i.e.,  $\pi_1$ contains $x_{j_2}$ and $x_{j_2} \neq x_k$, then let $\pi_1 = \pi_{1,1} \concat \pi_{1,2}$ such that $\pi_{1,1}$ is the prefix of $\pi_1$ that goes from $x_{j_1}$ to $x_{j_2}$. 

Let $\mathsf{Ineq}_{\pi_0 \concat e_1}$ be $x_{k} \ge d_0 + \sum_{j \in [n]} d_{j} x_j$. Then $d_{j_1} \ge 1$ and $d_{j_2} \ge 1$. Moreover, let $\mathsf{Ineq}_{\pi_{1,1}}$ be $x_{j_1} \ge d'_0 + \sum_{j \in [n]} d'_{j} x_j$. Then $d'_{j_2} \ge 1$. Hence $\mathsf{Ineq}_{\pi_0 \concat e_1 \concat \pi_{1,1}}$ is 
\[%\renewcommand{\arraystretch}{1.5}
\begin{array}{l l l}
x_k & \ge & d_0 + \sum_{j \in [n] \setminus \{j_1\}} d_{j} x_j + d_{j_1} (d'_0 + \sum_{j \in [n]} d'_{j} x_j)\\
& = & (d_0 + d_{j_1} d'_0) + \sum_{j \in [n] \setminus \{j_1\}} (d_{j} + d_{j_1}d'_j) x_j  + d_{j_1} d'_{j_1} x_{j_1}.
\end{array}
\]
From $d_{j_1} \ge 1$, $d_{j_2} \ge 1$ and $d'_{j_2} \ge 1$, we deduce that $d_{j_2} + d_{j_1}d'_{j_2} \ge 2$.
Consequently, in $\mathsf{Ineq}_{\pi'_1} = \mathsf{Ineq}_{\pi_0 \concat e_1 \concat \pi_{1,1} \concat \pi_{1,2}}$, which is obtained from $\mathsf{Ineq}_{\pi_0 \concat e_1 \concat \pi_{1,1}}$ by replacing $x_{j_2}$ with the right-hand side of $\mathsf{Ineq}_{\pi_{1,2}}$, the coefficient of $x_{k}$ is at least two, since the coefficient of $x_{j_2}$ in $\mathsf{Ineq}_{\pi_0 \concat e_1 \concat \pi_{1,1}}$ is $d_{j_2} + d_{j_1}d'_{j_2} \ge 2$. The result follows.
%\qed
\end{itemize}
% \end{proof}

% In fact, the inverse of the proposition also holds:

% \begin{proposition}
% Suppose that $G_\varphi$ is strongly connected.
% If $G_\varphi$ does not contain two distinct edges out of some vertex $x_i$ of the same label, nor contains any edge $(x_i, l, a, x_j)$ such that $a > 1$, then either $\varphi$ has no solution, or there is no upper bound to its solutions.
% \end{proposition}

% \begin{proof}

\medskip
% \noindent\underline{\bf ``If'' direction}.
\noindent\underline{``If'' direction}.
Suppose the values of the variables in every solution of $\varphi$ are upper-bounded by $B$. We prove by contradiction.

If $G_\varphi$ is nonexpansive, then  $G_\varphi$ does not contain two distinct edges out of some vertex $x_i$ with the same label, nor contains any edge $(x_i, l, a, x_j)$ such that $a > 1$. It means that the inequalities for all the vertices $x_i$ must be of the form $x_i \geq a'+ x_j$ for some constant $a'\in\intnum$. 

Since $\varphi$ is satisfiable, let
$(u_1, u_2, \ldots, u_n)$ be a solution of $\varphi$. Obviously, for any $C \in \natnum$, $(u_1 + C, u_2 + C, \ldots, u_n + C)$ is also a solution of $\varphi$. Thus, 
the values of the variables in every solution of $\varphi$ are \emph{not} upper-bounded by $B$.\qed
\end{proof}
